Object Contour and Edge Detection with RefineContourNet

A ResNet-based multi-path refinement CNN is used for object contour detection. For this task, we prioritise the effective utilization of the high-level abstraction capability of a ResNet, which leads to state-of-the-art results for edge detection. Keeping our focus in mind, we fuse the high, mid and low-level features in that specific order, which differs from many other approaches. It uses the tensor with the highest-levelled features as the starting point to combine it layer-by-layer with features of a lower abstraction level until it reaches the lowest level. We train this network on a modified PASCAL VOC 2012 dataset for object contour detection and evaluate on a refined PASCAL-val dataset reaching an excellent performance and an Optimal Dataset Scale (ODS) of 0.752. Furthermore, by fine-training on the BSDS500 dataset we reach state-of-the-art results for edge-detection with an ODS of 0.824.

==> CAIP - Cleaned - Big/citations <==
Do not forget Krähenbühl


SED semantic scholar

@article{Liu2018SemanticED,
  title={Semantic Edge Detection with Diverse Deep Supervision},
  author={Yun Liu and Ming-Ming Cheng and Jiawang Bian and Le Zhang and Peng-Tao Jiang and Yang Cao},
  journal={CoRR},
  year={2018},
  volume={abs/1804.02864}
}

Deep Boundaries
Iasonas Kokkinos, “Pushing the boundaries of boundary detection using deep learning”, International Conference on Learning Representations, 2016. 


High-for-Low and Low-for-High
@InProceedings{gberta_2015_ICCV,
author = {Gedas Bertasius and Jianbo Shi and Lorenzo Torresani},
title = {High-for-Low and Low-for-High:
Efficient Boundary Detection from Deep Object Features and its Applications to High-Level Vision},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {December},
year = {2015}
}

Learning to Predict Crisp Boundaries

@InProceedings{10.1007/978-3-030-01231-1_35,
author="Deng, Ruoxi
and Shen, Chunhua
and Liu, Shengjun
and Wang, Huibing
and Liu, Xinru",
editor="Ferrari, Vittorio
and Hebert, Martial
and Sminchisescu, Cristian
and Weiss, Yair",
title="Learning to Predict Crisp Boundaries",
booktitle="Computer Vision -- ECCV 2018",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="570--586",
abstract="Recent methods for boundary or edge detection built on Deep Convolutional Neural Networks (CNNs) typically suffer from the issue of predicted edges being thick and need post-processing to obtain crisp boundaries. Highly imbalanced categories of boundary versus background in training data is one of main reasons for the above problem. In this work, the aim is to make CNNs produce sharp boundaries without post-processing. We introduce a novel loss for boundary detection, which is very effective for classifying imbalanced data and allows CNNs to produce crisp boundaries. Moreover, we propose an end-to-end network which adopts the bottom-up/top-down architecture to tackle the task. The proposed network effectively leverages hierarchical features and produces pixel-accurate boundary mask, which is critical to reconstruct the edge map. Our experiments illustrate that directly making crisp prediction not only promotes the visual results of CNNs, but also achieves better results against the state-of-the-art on the BSDS500 dataset (ODS F-score of .815) and the NYU Depth dataset (ODS F-score of .762).",
isbn="978-3-030-01231-1"
}

Richer Conv Fea
@ARTICLE{8516362,
author={Y. {Liu} and M. {Cheng} and X. {Hu} and J. {Bian} and L. {Zhang} and X. {Bai} and J. {Tang}},
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
title={Richer Convolutional Features for Edge Detection},
year={2018},
volume={},
number={},
pages={1-1},
keywords={Image edge detection;Feature extraction;Computer vision;Detectors;Training;Computer architecture;Task analysis;Edge detection;deep learning;richer convolutional features},
doi={10.1109/TPAMI.2018.2878849},
ISSN={0162-8828},
month={},}

Semantic Contours from Inverse Detectors

@InProceedings{BharathICCV2011,
  author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
  title        = "Semantic Contours from Inverse Detectors",
  booktitle    = "International Conference on Computer Vision (ICCV)",
  year         = "2011",
}

@INPROCEEDINGS{6126343,
author={B. {Hariharan} and P. {Arbeláez} and L. {Bourdev} and S. {Maji} and J. {Malik}},
booktitle={2011 International Conference on Computer Vision},
title={Semantic contours from inverse detectors},
year={2011},
volume={},
number={},
pages={991-998},
keywords={image classification;object detection;semantic contour;inverse detector;category-specific object contour;real world image;generic object detector;bottom-up contour;Detectors;Semantics;Vectors;Feature extraction;Support vector machines;Head;Humans},
doi={10.1109/ICCV.2011.6126343},
ISSN={2380-7504},
month={Nov},}


Weakly Superviced
@INPROCEEDINGS{7780396,
author={A. {Khoreva} and R. {Benenson} and M. {Omran} and M. {Hein} and B. {Schiele}},
booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={Weakly Supervised Object Boundaries},
year={2016},
volume={},
number={},
pages={183-192},
keywords={edge detection;learning (artificial intelligence);object detection;object-specific boundary annotations;high-quality object boundaries;bounding box annotations;weakly supervised annotations;weakly supervised object boundary detection;Training;Detectors;Semantics;Noise measurement;Image segmentation;Image edge detection;Training data},
doi={10.1109/CVPR.2016.27},
ISSN={1063-6919},
month={June},}

CED

@ARTICLE{8485388,
author={Y. {Wang} and X. {Zhao} and Y. {Li} and K. {Huang}},
journal={IEEE Transactions on Image Processing},
title={Deep Crisp Boundaries: From Boundaries to Higher-Level Tasks},
year={2019},
volume={28},
number={3},
pages={1285-1298},
keywords={computer vision;convolution;edge detection;feature extraction;image representation;image segmentation;image sequences;learning (artificial intelligence);object detection;higher-level tasks;edge detection;deep convolutional networks;ConvNet-based edge detectors;human level performance;standard benchmarks;edge pixels;crisp edge inputs;crisp edge detector;backward refinement pathway;human accuracy;deep crisp boundaries;object proposal generation;crisp edge maps;standard criteria;Image edge detection;Detectors;Task analysis;Proposals;Optical imaging;Semantics;Standards;Boundary detection;deep learning},
doi={10.1109/TIP.2018.2874279},
ISSN={1057-7149},
month={March},}


COB

@article{Maninis2017,
  author = {K.K. Maninis and J. Pont-Tuset and P. Arbel\'{a}ez and L. Van Gool},
  title = {Convolutional Oriented Boundaries: From Image Segmentation to High-Level Tasks},
  journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  year = {2017},
  volume = {40},
  number = {4},
  pages = {819 - 833}
}


CaseNet
@INPROCEEDINGS{8099674,
author={Z. {Yu} and C. {Feng} and M. {Liu} and S. {Ramalingam}},
booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={CASENet: Deep Category-Aware Semantic Edge Detection},
year={2017},
volume={},
number={},
pages={1761-1770},
keywords={computer vision;edge detection;image fusion;learning (artificial intelligence);semantic networks;skip-layer architecture;category-wise edge activations;deep category-aware semantic edge detection;edge cues;vision tasks;deep learning;classical edge detection;challenging multilabel problem;edge pixel;semantic classes;end-to-end deep semantic edge detection;multi-label loss function;end-to-end deep semantic edge learning architecture;Image edge detection;Semantics;Computer architecture;Convolution;Feature extraction;Image color analysis},
doi={10.1109/CVPR.2017.191},
ISSN={1063-6919},
month={July},}


ObjContDet

@INPROCEEDINGS{7780397,
author={J. {Yang} and B. {Price} and S. {Cohen} and H. {Lee} and M. {Yang}},
booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={Object Contour Detection with a Fully Convolutional Encoder-Decoder Network},
year={2016},
volume={},
number={},
pages={193-202},
keywords={combinatorial mathematics;image coding;image matching;image segmentation;learning (artificial intelligence);object detection;fully-convolutional encoder-decoder network;deep learning algorithm;higher-level object contour detection;PASCAL VOC;refined ground truth;polygon annotations;object classes;MS COCO;edge detection;BSDS500;image matching;multiscale combinatorial grouping algorithm;high-quality segmented object;average recall improvement;Training;Decoding;Image edge detection;Proposals;Image segmentation;Semantics;Labeling},
doi={10.1109/CVPR.2016.28},
ISSN={1063-6919},
month={June},}


HED

@INPROCEEDINGS{7410521,
author={S. {Xie} and Z. {Tu}},
booktitle={2015 IEEE International Conference on Computer Vision (ICCV)},
title={Holistically-Nested Edge Detection},
year={2015},
volume={},
number={},
pages={1395-1403},
keywords={edge detection;feature extraction;feedforward neural nets;image classification;image representation;image resolution;learning (artificial intelligence);holistically-nested edge detection algorithm;holistic image training;multiscale feature learning;pixel-wise edge classification;image-to-image prediction;deep learning model;convolutional neural networks;deeply-supervised nets;hierarchical representations;object boundary detection;BSD500 dataset;NYU Depth dataset;Image edge detection;Training;Neural networks;Detectors;Feature extraction;Machine learning;Predictive models},
doi={10.1109/ICCV.2015.164},
ISSN={2380-7504},
month={Dec},}



==> citations <==
Do not forget Krähenbühl


SED semantic scholar

@article{Liu2018SemanticED,
  title={Semantic Edge Detection with Diverse Deep Supervision},
  author={Yun Liu and Ming-Ming Cheng and Jiawang Bian and Le Zhang and Peng-Tao Jiang and Yang Cao},
  journal={CoRR},
  year={2018},
  volume={abs/1804.02864}
}

Deep Boundaries
Iasonas Kokkinos, “Pushing the boundaries of boundary detection using deep learning”, International Conference on Learning Representations, 2016. 


High-for-Low and Low-for-High
@InProceedings{gberta_2015_ICCV,
author = {Gedas Bertasius and Jianbo Shi and Lorenzo Torresani},
title = {High-for-Low and Low-for-High:
Efficient Boundary Detection from Deep Object Features and its Applications to High-Level Vision},
booktitle = {The IEEE International Conference on Computer Vision (ICCV)},
month = {December},
year = {2015}
}

Learning to Predict Crisp Boundaries

@InProceedings{10.1007/978-3-030-01231-1_35,
author="Deng, Ruoxi
and Shen, Chunhua
and Liu, Shengjun
and Wang, Huibing
and Liu, Xinru",
editor="Ferrari, Vittorio
and Hebert, Martial
and Sminchisescu, Cristian
and Weiss, Yair",
title="Learning to Predict Crisp Boundaries",
booktitle="Computer Vision -- ECCV 2018",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="570--586",
abstract="Recent methods for boundary or edge detection built on Deep Convolutional Neural Networks (CNNs) typically suffer from the issue of predicted edges being thick and need post-processing to obtain crisp boundaries. Highly imbalanced categories of boundary versus background in training data is one of main reasons for the above problem. In this work, the aim is to make CNNs produce sharp boundaries without post-processing. We introduce a novel loss for boundary detection, which is very effective for classifying imbalanced data and allows CNNs to produce crisp boundaries. Moreover, we propose an end-to-end network which adopts the bottom-up/top-down architecture to tackle the task. The proposed network effectively leverages hierarchical features and produces pixel-accurate boundary mask, which is critical to reconstruct the edge map. Our experiments illustrate that directly making crisp prediction not only promotes the visual results of CNNs, but also achieves better results against the state-of-the-art on the BSDS500 dataset (ODS F-score of .815) and the NYU Depth dataset (ODS F-score of .762).",
isbn="978-3-030-01231-1"
}

Richer Conv Fea
@ARTICLE{8516362,
author={Y. {Liu} and M. {Cheng} and X. {Hu} and J. {Bian} and L. {Zhang} and X. {Bai} and J. {Tang}},
journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
title={Richer Convolutional Features for Edge Detection},
year={2018},
volume={},
number={},
pages={1-1},
keywords={Image edge detection;Feature extraction;Computer vision;Detectors;Training;Computer architecture;Task analysis;Edge detection;deep learning;richer convolutional features},
doi={10.1109/TPAMI.2018.2878849},
ISSN={0162-8828},
month={},}

Semantic Contours from Inverse Detectors

@InProceedings{BharathICCV2011,
  author       = "Bharath Hariharan and Pablo Arbelaez and Lubomir Bourdev and Subhransu Maji and Jitendra Malik",
  title        = "Semantic Contours from Inverse Detectors",
  booktitle    = "International Conference on Computer Vision (ICCV)",
  year         = "2011",
}

@INPROCEEDINGS{6126343,
author={B. {Hariharan} and P. {Arbeláez} and L. {Bourdev} and S. {Maji} and J. {Malik}},
booktitle={2011 International Conference on Computer Vision},
title={Semantic contours from inverse detectors},
year={2011},
volume={},
number={},
pages={991-998},
keywords={image classification;object detection;semantic contour;inverse detector;category-specific object contour;real world image;generic object detector;bottom-up contour;Detectors;Semantics;Vectors;Feature extraction;Support vector machines;Head;Humans},
doi={10.1109/ICCV.2011.6126343},
ISSN={2380-7504},
month={Nov},}


Weakly Superviced
@INPROCEEDINGS{7780396,
author={A. {Khoreva} and R. {Benenson} and M. {Omran} and M. {Hein} and B. {Schiele}},
booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={Weakly Supervised Object Boundaries},
year={2016},
volume={},
number={},
pages={183-192},
keywords={edge detection;learning (artificial intelligence);object detection;object-specific boundary annotations;high-quality object boundaries;bounding box annotations;weakly supervised annotations;weakly supervised object boundary detection;Training;Detectors;Semantics;Noise measurement;Image segmentation;Image edge detection;Training data},
doi={10.1109/CVPR.2016.27},
ISSN={1063-6919},
month={June},}

CED

@ARTICLE{8485388,
author={Y. {Wang} and X. {Zhao} and Y. {Li} and K. {Huang}},
journal={IEEE Transactions on Image Processing},
title={Deep Crisp Boundaries: From Boundaries to Higher-Level Tasks},
year={2019},
volume={28},
number={3},
pages={1285-1298},
keywords={computer vision;convolution;edge detection;feature extraction;image representation;image segmentation;image sequences;learning (artificial intelligence);object detection;higher-level tasks;edge detection;deep convolutional networks;ConvNet-based edge detectors;human level performance;standard benchmarks;edge pixels;crisp edge inputs;crisp edge detector;backward refinement pathway;human accuracy;deep crisp boundaries;object proposal generation;crisp edge maps;standard criteria;Image edge detection;Detectors;Task analysis;Proposals;Optical imaging;Semantics;Standards;Boundary detection;deep learning},
doi={10.1109/TIP.2018.2874279},
ISSN={1057-7149},
month={March},}


COB

@article{Maninis2017,
  author = {K.K. Maninis and J. Pont-Tuset and P. Arbel\'{a}ez and L. Van Gool},
  title = {Convolutional Oriented Boundaries: From Image Segmentation to High-Level Tasks},
  journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)},
  year = {2017},
  volume = {40},
  number = {4},
  pages = {819 - 833}
}


CaseNet
@INPROCEEDINGS{8099674,
author={Z. {Yu} and C. {Feng} and M. {Liu} and S. {Ramalingam}},
booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={CASENet: Deep Category-Aware Semantic Edge Detection},
year={2017},
volume={},
number={},
pages={1761-1770},
keywords={computer vision;edge detection;image fusion;learning (artificial intelligence);semantic networks;skip-layer architecture;category-wise edge activations;deep category-aware semantic edge detection;edge cues;vision tasks;deep learning;classical edge detection;challenging multilabel problem;edge pixel;semantic classes;end-to-end deep semantic edge detection;multi-label loss function;end-to-end deep semantic edge learning architecture;Image edge detection;Semantics;Computer architecture;Convolution;Feature extraction;Image color analysis},
doi={10.1109/CVPR.2017.191},
ISSN={1063-6919},
month={July},}


ObjContDet

@INPROCEEDINGS{7780397,
author={J. {Yang} and B. {Price} and S. {Cohen} and H. {Lee} and M. {Yang}},
booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title={Object Contour Detection with a Fully Convolutional Encoder-Decoder Network},
year={2016},
volume={},
number={},
pages={193-202},
keywords={combinatorial mathematics;image coding;image matching;image segmentation;learning (artificial intelligence);object detection;fully-convolutional encoder-decoder network;deep learning algorithm;higher-level object contour detection;PASCAL VOC;refined ground truth;polygon annotations;object classes;MS COCO;edge detection;BSDS500;image matching;multiscale combinatorial grouping algorithm;high-quality segmented object;average recall improvement;Training;Decoding;Image edge detection;Proposals;Image segmentation;Semantics;Labeling},
doi={10.1109/CVPR.2016.28},
ISSN={1063-6919},
month={June},}


HED

@INPROCEEDINGS{7410521,
author={S. {Xie} and Z. {Tu}},
booktitle={2015 IEEE International Conference on Computer Vision (ICCV)},
title={Holistically-Nested Edge Detection},
year={2015},
volume={},
number={},
pages={1395-1403},
keywords={edge detection;feature extraction;feedforward neural nets;image classification;image representation;image resolution;learning (artificial intelligence);holistically-nested edge detection algorithm;holistic image training;multiscale feature learning;pixel-wise edge classification;image-to-image prediction;deep learning model;convolutional neural networks;deeply-supervised nets;hierarchical representations;object boundary detection;BSD500 dataset;NYU Depth dataset;Image edge detection;Training;Neural networks;Detectors;Feature extraction;Machine learning;Predictive models},
doi={10.1109/ICCV.2015.164},
ISSN={2380-7504},
month={Dec},}


